Distribution-Aware Prompt Tuning for Vision-Language Models

Pre-trained vision-language models (VLMs) have shown impressive performance on various downstream tasks by utilizing knowledge learned from large data. In general, the performance of VLMs on target tasks can be further improved by prompt tuning, which adds context to the input image or text. By leveraging data from target tasks, various prompt-tuning methods have been studied in the literature. A key to prompt tuning is the feature space alignment between two modalities via learnable vectors with model parameters fixed. We observed that the alignment becomes more effective when embeddings of each modality are `well-arranged' in the latent space. Inspired by this observation, we proposed distribution-aware prompt tuning (DAPT) for vision-language models, which is simple yet effective. Specifically, the prompts are learned by maximizing inter-dispersion, the distance between classes, as well as minimizing the intra-dispersion measured by the distance between embeddings from the same class. Our extensive experiments on 11 benchmark datasets demonstrate that our method significantly improves generalizability. The code is available at https://github.com/mlvlab/DAPT.

==> 4.experiment_bk.tex <==
\section{Experiments}
\label{s:exp}
\noindent\textbf{Datasets. } 
We evaluate DAPT on few-shot image classification and domain generalization settings. 
We evaluate 11 public datasets in few-shot learning, 
Food101~\cite{bossard2014food}, 
DTD~\cite{cimpoi2014describing}, 
Imagenet~\cite{deng2009imagenet}, 
Caltech101~\cite{fei2004learning}, 
EuroSAT~\cite{helber2019eurosat}, 
StanfordCars~\cite{krause20133d}, 
FGVCAircraft~\cite{maji13fine-grained}, 
Flowers102~\cite{nilsback2008automated}, 
OxfordPets~\cite{parkhi2012cats}, 
UCF101~\cite{soomro2012ucf101}, 
and SUN397~\cite{xiao2010sun}, using 1, 2, 4, 8, and 16-shots per dataset. 
In the domain generalization setting, we set the source dataset to ImageNet and test to target dataset - ImageNet-R~\cite{hendrycks2021many}, ImageNet-A~\cite{hendrycks2021natural},  ImageNetV2~\cite{recht2019imagenet}, and ImageNet-Sketch~\cite{wang2019learning}. 

\noindent\textbf{Baselines. }
In the experiments, we compare with zero-shot CLIP, linear probe CLIP, CoOp~\cite{zhou2022coop}, and VPT~\cite{jia2022visual}. 
In the case of zero-shot CLIP, we test with pre-trained CLIP without additional training. 
On the other hand, we fine-tune the classifier in the case of linear probe CLIP following Radford \etal~\cite{radford2021learning}. 
Because we demonstrate DAPT on CLIP with the ViT-B/16 image encoder backbone, we implement CoOp and VPT with ViT-B/16. 
Additionally, we observed that VPT has various accuracy gaps in the few-shot learning setting. 
For a fair comparison, we search hyperparameters (\textit{i.e.}, learning rate) with ranges from 0.002 to 20, as reported in Table~\ref{tab:vpt_lr}. 
The figures show the average accuracy of 11 datasets in 16-shots image classification settings for each learning rate. 
As a result, we set the learning rate is 0.2 on VPT in all experiments. 

\input{tables/lr_ablation}
\noindent\textbf{Implementation Details. }
We use pre-trained CLIP~\cite{radford2021learning} with ViT-B/16 image encoder backbone from the official repository\footnote{https://github.com/openai/CLIP}. 
To construct prompts for text and visual encoders, we refer to CoOp and VPT open sources\footnote{https://github.com/KaiyangZhou/CoOp}$^{,}$\footnote{https://github.com/KMnP/vpt}. 
In all experiments, we evaluate three times on NVIDIA RTX-3090 GPUs and report the average value.  
More implementation details are included in the supplement. 

\subsection{Few-Shot Learning}
Figure~\ref{fig:graph} summarizes the performance of DAPT in few-shot learning on 11 datasets and the average accuracy.
Each plot compares DAPT with baselines. 
The experiments show DAPT outperforms baselines on most benchmark datasets. 
In addition, Figure~\ref{fig:bar} also shows that DAPT consistently outperforms revious prompt tuning methods - CoOp~\cite{zhou2022coop} and VPT~\cite{jia2022visual} on all datasets. 

\input{tables/lpclip_1shot}
\input{figs/fig_zsclip}
\noindent\textbf{Comparison with Linear Probe CLIP. }
We observed that DAPT shows higher performance than linear probe CLIP for most datasets as noted in Table~\ref{tab:lpclip_1shot}. 
Especially on OxfordPets~\cite{parkhi2012cats}, DAPT improves the performance by 46.22\% with only a single training sample. 
When comparing all experiments in 1-shot image classification, DAPT achieves an average improvement of 14.87\% compared to linear probe CLIP. 

\noindent\textbf{Comparison with Zero-Shot CLIP. }
When comparing DAPT to zero-shot CLIP, DAPT demonstrates higher performance in most experiments, with a similar result to the comparison with linear probe CLIP. 
Notably, as described in Figure~\ref{fig:zsclip}, the performance gap between DAPT and zero-shot CLIP widens as the number of samples increases, suggesting that DAPT is adaptive at distribution-aware prompt optimization as the training sample size grows.

\input{figs/fig_graph}
\input{figs/fig_bar}

\noindent\textbf{Comparison with Previous Prompt Tuning. }
Figure~\ref{fig:bar_coop} demonstrates the results of DAPT and CoOp~\cite{zhou2022coop} on 16 shots. 
As shown in the results, DAPT outperforms CoOp for all datasets. Furthermore, Figure~\ref{fig:bar_vpt} presents the comparison of DAPT and VPT~\cite{jia2022visual} under the same experimental setting. 
As with the CoOp comparison results, it shows that DAPT outperforms VPT on all datasets, and the accuracy is 12.43\% higher than VPT on StanfordCars~\cite{krause20133d}.
To sum up, using DAPT for each modality shows superior performance compared to conventional prompt tuning, as well as zero-shot CLIP and liner probe CLIP.

\subsection{Domain Generalization}
We evaluate the generalizability of DAPT by comparing it with zero-shot CLIP, and linear probe CLIP in the domain generalization setting. 
We use ImageNet~\cite{deng2009imagenet} as a source dataset,and the prompts are trained with 16 samples and the target dataset as ImageNet-R~\cite{hendrycks2021many}, ImageNet-A~\cite{hendrycks2021natural}, ImageNetV2~\cite{recht2019imagenet}, and ImageNet-Sketch~\cite{wang2019learning}. 
\input{tables/imagenet_generalization}
\noindent The overall results are shown in Table~\ref{tab:imagenet_generalization}. 
From the experimental results, DAPT achieves remarkable performance on unseen data compared to zero-shot CLIP and linear probe CLIP. 
Compared with CoOp~\cite{zhou2022coop} and VPT~\cite{jia2022visual}, it slightly decreases accuracy on ImageNet-A and ImageNet-R, respectively. In contrast, in the rest of the dataset, ImageNet-V2 and ImageNet-Sketch, DAPT has superior performance with a significant accuracy gain.

\subsection{Ablation Study}
\noindent\textbf{Effectiveness of Intra-dispersion Loss and Inter-dispersion Loss. } 
To verify the accuracy improvement when applying the inter-dispersion loss and intra-dispersion loss, we test few-shot learning experiments on 11 datasets with 16 samples from training data. 
We set the model combined with text prompts, \textit{i.e.}, CoOp~\cite{zhou2022coop}, and visual prompts, \textit{i.e.}, VPT~\cite{jia2022visual}, as a baseline. 
Table~\ref{tab:ablation_loss} shows the performance improvement of applying inter-dispersion loss and intra-dispersion loss. 
The experimental results indicate that the accuracy improved overall for 11 datasets and the average of the entire datasets compared to the baseline. 
As a result, both inter-dispersion loss and intra-dispersion loss show performance gain by reconstructing the embedding space across most datasets. 
In particular, the inter-dispersion loss and intra-dispersion loss are effective for improving performance on FGVCAircraft~\cite{maji13fine-grained}, and DTD~\cite{cimpoi2014describing}, respectively. 
Interestingly, despite some datasets, \textit{i.e.}, Food101~\cite{bossard2014food}, ImageNet~\cite{deng2009imagenet}, FGVCAircraft~\cite{maji13fine-grained}, Flowers102~\cite{nilsback2008automated}, and SUN397~\cite{xiao2010sun}, slightly decreasing accuracy by adding inter-dispersion loss or intra-dispersion loss, DAPT increases accuracy. 
\input{tables/ablation_shots}
The results support that reconstructing and optimizing embedding jointly are essential to feature alignment between the modalities. 
As noted in Table~\ref{tab:ablation_shots}, this tendency can also be observed for various shots - DAPT has superior performance compared with the combination of CoOp~\cite{zhou2022coop} and VPT~\cite{jia2022visual}. 

\input{tables/ablation_dispersion}

\noindent\textbf{Exploration of Intra-dispersion Loss. }
As discussed in Section~\ref{s:method}, the prototype $\boldsymbol{s}$ is defined as the average of image embeddings in DAPT. 
To evaluate the prototypes set by the mean of embeddings,
we conduct the ablation study of intra-dispersion loss with the prototype (DAPT-R) set by a random sample's embedding. 
Table~\ref{tab:ablation_uniform} shows the image classification results for 1, 2, 4, 8, and 16-shots on 11 datasets.
From the results, we confirmed that clustering around the average of samples (DAPT) is more effective than clustering around the random sample (DAPT-R),
especially when the number of shots is not extremely small (\textit{i.e.}, 4, 8, and 16-shots). 
\input{tables/ablation_uniform} 

\subsection{Analysis}
We investigate whether DAPT learns text and image embeddings as intended - spreading text embeddings and assembling image embeddings within the same classes - by quantitative and qualitative analyses. 

\noindent\textbf{Quantitative Analysis. }
\noindent We analyze the pairwise distance $\text{pdist}$ and the area of the convex hull of embeddings. 
Table~\ref{tab:numerical_pairwise_distance} shows the relative average pairwise distance $\text{pdist}$ between image embeddings of the same class compared to zero-shot CLIP, which is computed as the relative ratios, \ie, $\Delta \text{pdist (\%)}  = (1-\text{DAPT}/\text{zero-shot CLIP})\times 100$.
The results evidence that DAPT properly minimizes the average pairwise distance between image embeddings in a class ($\approx$ intra-dispersion)
and maximizes it for text (labels) embeddings across classes ($\approx$ inter-dispersion).
This implies that DAPT learns prompts to better latent spaces for feature alignment.

\input{tables/numerical}
\noindent\textbf{Qualitative Analysis. }
We verify that DAPT more compactly clusters image embeddings via t-SNE~\cite{van2008visualizing} visualization on several datasets. 
Figure~\ref{fig:qual} shows image embeddings of Fowers102~\cite{nilsback2008automated} and UCF101~\cite{soomro2012ucf101} benchmark datasets. 
Each point represents an image embedding, and the colors of the points indicate their classes. 
More t-SNE visualizations are provided in the supplement. 

\input{figs/fig_qual}
